Characterizing physiological and symptomatic variation in menstrual cycles using self-tracked mobile health data

The menstrual cycle is a key indicator of overall health for women of reproductive age. Previously, menstruation was primarily studied through survey results; however, as menstrual tracking mobile apps become more widely adopted, they provide an increasingly large, content-rich source of menstrual health experiences and behaviors over time. By exploring a database of user-tracked observations from the Clue app by BioWink of over 378,000 users and 4.9 million natural cycles, we show that self-reported menstrual tracker data can reveal statistically significant relationships between per-person cycle length variability and self-reported qualitative symptoms. A concern for self-tracked data is that they reflect not only physiological behaviors, but also the engagement dynamics of app users. To mitigate such potential artifacts, we develop a procedure to exclude cycles lacking user engagement, thereby allowing us to better distinguish true menstrual patterns from tracking anomalies. We uncover that women located at different ends of the menstrual variability spectrum, based on the consistency of their cycle length statistics, exhibit statistically significant differences in their cycle characteristics and symptom tracking patterns. We also find that cycle and period length statistics are stationary over the app usage timeline across the variability spectrum. The symptoms that we identify as showing statistically significant association with timing data can be useful to clinicians and users for predicting cycle variability from symptoms or as potential health indicators for conditions like endometriosis. Our findings showcase the potential of longitudinal, high-resolution self-tracked data to improve understanding of menstruation and women's health as a whole.

==> tables/tab_interesting_low_high_extremes.tex <==
% Table for categories and symptoms
\begin{table*}
\caption{Pain and period tracking odds ratios for low extreme end of the proportion range}
\label{tab:interesting_low_extremes}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\cline{1-5}
Category & Symptom & Consistently highly variable group's likelihood for $\lambda_s < 0.05$ (95\% CI) & Consistently not highly variable group's likelihood for $\lambda_s < 0.05$ (95\% CI) & Odds ratio (95\% CI) for $\lambda_s < 0.05$ \\ \cline{1-5}
Period flow&heavy&0.170 (0.169,0.170) &0.098 (0.096,0.100) &1.734 (1.703,1.766) \\ \hdashline
Period flow&spotting&0.314 (0.313,0.315) & 0.239 (0.237,0.241) &1.314 (1.300,1.328) \\ \hdashline
Type of pain experienced&headache&0.326 (0.325,0.327) &0.269 (0.266,0.272) &1.212 (1.199,1.225)  \\ \hdashline
Type of pain experienced&tender breasts&0.366 (0.365,0.367) &0.320 (0.317,0.322) &1.145 (1.134,1.156) \\
\cline{1-5}
\end{tabular}
\end{center}
	Likelihood of low $\lambda_s$ per group, with the associated odds ratio (and 95\% confidence intervals). The probability of not tracking `heavy period' for users in the consistently highly variable group is 0.17 and 0.098 in the other, with an odds ratio of 1.734: the consistently highly variable is more likely not to track `heavy period'.

\vspace*{5ex}
\caption{Pain and period tracking odds ratios for high extreme end of the proportion range}
\label{tab:interesting_high_extremes}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
	\cline{1-5}
	Category & Symptom & Consistently highly variable group's likelihood for $\lambda_s> 0.95$ & Consistently not highly variable group's likelihood for $\lambda_s> 0.95$ &  Odds ratio (95\% CI) for $\lambda_s> 0.95$ \\ \cline{1-5}
Period flow&heavy& 0.078 (0.077,0.079) & 0.096 (0.094,0.097) &0.817 (0.802,0.833) \\ \hdashline
Period flow&spotting& 0.067 (0.066,0.067) &0.039 (0.037,0.040) &1.729 (1.679,1.782) \\ \hdashline
Type of pain experienced&tender breasts& 0.193 (0.192,0.194) &0.113 (0.111,0.115) & 1.715 (1.684,1.746) \\ \hdashline
Type of pain experienced&headache& 0.218 (0.217,0.219) &0.131 (0.129,0.133) &1.663 (1.636,1.691) \\
	\cline{1-5}
\end{tabular}
\end{center}
Likelihood of high $\lambda_s$ per group, with the associated odds ratio (and 95\% confidence intervals). The probability of consistently tracking `tender breast' pain for users in the consistently highly variable group is 0.193 and 0.113 in the other, with an odds ratio of 1.715: the consistently highly variable is more likely to regularly track  `tender breast' pain.
\end{table*}
